Physically Aware Synthesis Revisited: Guiding Technology Mapping with Primitive Logic Gate Placement

A typical VLSI design flow is divided into separated front-end logic synthesis and back-end physical design (PD) stages, which often require costly iterations between these stages to achieve design closure. Existing approaches face significant challenges, notably in utilizing feedback from physical metrics to better adapt and refine synthesis operations, and in establishing a unified and comprehensive metric. This paper introduces a new Primitive logic gate placement guided technology MAPping (PigMAP) framework to address these challenges. With approximating technology-independent spatial information, we develop a novel wirelength (WL) driven mapping algorithm to produce PD-friendly netlists. PigMAP is equipped with two schemes: a performance mode that focuses on optimizing the critical path WL to achieve high performance, and a power mode that aims to minimize the total WL, resulting in balanced power and performance outcomes. We evaluate our framework using the EPFL benchmark suites with ASAP7 technology, using the OpenROAD tool for place-and-route. Compared with OpenROAD flow scripts, performance mode reduces delay by 14% while increasing power consumption by only 6%. Meanwhile, power mode achieves a 3% improvement in delay and a 9% reduction in power consumption.

==> attemps/method.tex <==
\section{Methodology}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\label{sec:method}
pigMAP, standing for the {\bf p}rimitive log{\bf i}c {\bf g}ate placement guided technology {\bf MAP}ping, employs wirelength constraints to direct an efficient mapping search, significantly enhancing the correlation between logic synthesis and the final routed design. 
By doing so, pigMAP achieves remarkable improvements in reducing both critical path delays and power consumption.
In this section, we first outline the overall flow of the pigMAP framework and compare it with the conventional flow (Section~\ref{subsec:of}). 
After providing an overarching introduction, we delve into the specifics of AIG placement implementation in Section~\ref{subsec:ap}. 
Finally, we detail our flow and its two optional mapping strategies: one focused on reducing delay and the other on improving power consumption (Section~\ref{subsec:pigMAP}).

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{algorithm}[t]
    \caption{pigMAP Flow}
    \label{alg:pigMAP}
    \begin{algorithmic}[1]
    \REQUIRE Logic network AIG $\mathbb{A}$ and mapping strategy $\mathbb{S}$
    \ENSURE Gate-level netlist
    \STATE Initialize data structure of mapping $\mathbb{M}$;
    \STATE Compute and match cuts $\mathbb{C}$, and initialize pins $\mathbb{P}$;
    \STATE All node position $\mathbb{N} \leftarrow$ \texttt{Placer}($\mathbb{A}$); {\hfill//Algorithm~\ref{alg:aigplace}}
    \FORALL{node $n$ in $\mathbb{A}$}
        \FORALL{$cut$ in $\mathbb{C}$}
            \STATE $\mathbb{P}_n \leftarrow$ \texttt{searchPin}($cut$); {\hfill//Algorithm~\ref{alg:search_pins}}
        \ENDFOR
    \ENDFOR
    \STATE $\mathbb{M} \leftarrow$ \texttt{delayMap}($\mathbb{A}, \mathbb{C}$); {\hfill//Execute mapping}
    \STATE Get global time constraint $\mathcal{C}_{t}$;
    \STATE $\mathbb{M} \leftarrow$ \texttt{globalAreaMap}($\mathbb{A}, \mathbb{C}, \mathcal{C}_{t}$);
    \STATE Update global time constraint $\mathcal{C}_{t}$;
    \IF{$\mathbb{S}$ == pigMAP-Power} 
        \STATE $\mathbb{M} \leftarrow$ \texttt{pigMAP\_power}($\mathbb{A}, \mathbb{C}, \mathcal{C}_{t}, \mathbb{N}, \mathbb{P}$);
        \STATE Get global wirelength constraint $\mathcal{C}_{w_t}$;
    \ELSE
        \STATE $\mathbb{M} \leftarrow$ \texttt{pigMAP\_performance}($\mathbb{A}, \mathbb{C}, \mathcal{C}_{t}, \mathbb{N}, \mathbb{P}$);
        \STATE Get critical path wirelength constraint $\mathcal{C}_{w_c}$;
    \ENDIF
    \STATE $\mathbb{M} \leftarrow$ \texttt{detailAreaMap}($\mathbb{A}, \mathbb{C}, \mathcal{C}_{t}, \mathcal{C}_{w_t}, \mathcal{C}_{w_c}$);
    \RETURN \texttt{genNetlist}($\mathbb{M}$);
    \end{algorithmic}
\end{algorithm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Overall flow}
\label{subsec:of}
Fig.~\ref{fig:patmflow} and Algorithm~\ref{alg:pigMAP} illustrate the architecture of our proposed methodology. Highlighted by red cubes, our pigMAP framework consists of two main components: pigMAP-AIG Placer and pigMAP-Mapper. 
The processes involved in these components are detailed as follows:

{\bf 1. pigMAP-AIG Placer.}
The pigMAP-AIG Placer, as outlined in Algorithm~\ref{alg:aigplace}, begins with conducting a simulated floorplan over the input AIG. 
An approximate placement is then performed to determine the approximate position of each AIG node. 
After the placement, the mapper gets the nodes in the AIG and their approximate positions sequentially.

{\bf 2. pigMAP-Mapper.} 
The pigMAP-Mapper procedure first selects supergates that suit the corresponding cut function from the cell library and initializes parameters for each node. 
For each node in an AIG, pigMAP-Mapper enumerates all available cuts and supergates to search for their ``pins'', defined as the parent nodes of cut leaves in our algorithm.
The search for pins begins with the root of cut $c_i$ and recursively visits its children to determine if they are leaves (Algorithm~\ref{alg:search_pins}). 
Once a child is confirmed as a leaf, its parent node is recognized as a pin and added to the pin set of $c_i$.
Additionally the root is also considered a pin.
% \textcolor{red}{(``also'' sounds weird, just directly says Roots are defined/considered as pins.)}.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{algorithm}[t]
    \caption{Function \texttt{searchPin}().}
    \label{alg:search_pins}
    \begin{algorithmic}[1]
    \REQUIRE node $n$, cut $cut$, and level of search depth $l=0$
    \ENSURE pins $\mathbb{P}$
    \IF{$l$ > limit level of search depth $limit$}
        \RETURN $\mathbb{P}$;
    \ENDIF
    \STATE $l \gets l + 1$;
    \IF{size($cut$) == 0}
        \STATE $\mathbb{P} \leftarrow$ root of $cut$;
    \ENDIF
    \FORALL{fanin $child$ of $n$}
        \STATE $in\_cut \gets false$;
        \IF{$child$ in $cut$}
            \STATE $in\_cut \gets true$;
            \STATE break;
        \ENDIF
        \IF{$in\_cut == false$}
            \IF{$l > limit - 1$}
                \STATE $\mathbb{P} \leftarrow$ $child$;
                \RETURN $\mathbb{P}$;
            \ENDIF 
            \STATE $\mathbb{P} \leftarrow$ \texttt{searchPin}($child$, $cut$, $l$);
            \ELSE
                \RETURN $\mathbb{P}$;
        \ENDIF
    \ENDFOR
    \end{algorithmic}
\end{algorithm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{ownexample}
\label{exam0}
    For instance, consider an AIG with five PIs ($1, 2, 3, 4, 5$), two POs ($po1, po2$), and six intermediate nodes ($6, 7, 8, 9, 10, 11$), as depicted in Fig.\ref{fig:aig1}. 
    For node $8$, two different cuts are identified: \{$2,7$\} and \{$2,3,4$\}.
    Each cut has associated pins: the cut \{$2,7$\} is associated with the pin \{$8$\} and the cut \{$2,3,4$\} has pins \{$7,8$\}.
\end{ownexample}


Following the initial setup, the pigMAP-Mapper utilizes a delay-driven and global area-driven approach to process the input AIG, similar to conventional mapping workflows. 
After each mapping iteration, delay constraints are updated to maintain timing estimation.
% \textcolor{red}{(what do you mean by optimizing other metrics while "updating/recalculating"? It seems to me that is not reasonable to do them together)while optimizing other performance metrics.}
Under timing constraints, pigMAP-Mapper further perform two optimization iterations of a wirelength-driven mapping flow, specifically aiming to minimizing the wirelength of the final mapped netlist. 
During the wirelength-driven mapping \textcolor{red}{confirmed} phase, two alternative \textcolor{red}{confirmed} refinement strategies are available: performance-driven mapping (\textbf{pigMAP-Performance}), which focuses on the critical path wirelength, and power-driven mapping (\textbf{pigMAP-Power}), which targets a reduction in overall global wirelength.
After these strategic iterations, pigMAP-Mapper utilizes two rounds of a heuristic detailed area optimizations to further minimize the area of the final mapped netlist.
% \textcolor{red}{(cannot understand, why traversal is required to "complate" the mapping, what does "complete" means?)}
With resultant mapping solution given by mapping flow, \texttt{genNetlist} cover the AIG from POs to PIs through visiting leaves and combining the ``best supergate'' saved in each visited gate, generating the final netlist. 

% \textcolor{red}{(which step?) This step} ensures that each node is \textcolor{red}{(can you ``ensure'' optimality? if not, be careful about absolute words)optimally} mapped according to the refined constraints and metrics, finalizing the mapping solution and preparing the resultant netlist for physical design submission.

% \textcolor{red}{The rest of the section gives an detailed description of the algorithm.
% In Sec. XXX, aaaa
% In Sec. yyy, bbb...}
The remainder of this section gives an detailed description of the algorithm.
In Sec.~\ref{subsec:ap}, we illuminate primitive logic gate placement.
In Sec.~\ref{subsec:pigMAP}, we illuminate detailed mapping process of pigMAP and its two distinct model formulated for performance and power optimization.

\subsection{pigMAP-Placer: primitive logic gate placement}
\label{subsec:ap}
% Modern analytical placers view the placement problem as a nonlinear optimization challenge, often resulting in lengthy iteration times. 
% To accelerate the placement process, we use a graph convolution-based placer to efficiently produce optimized placement results. 
% This placer is an in-house version similar to the work~\cite{graphplanner}. 
% Specifically, the optimization objective for the approximate placement is to minimize total wirelength while reducing overlap, which in essence is to construct an optimized mapping from circuit connectivity to physical locations of nodes. 
% To this end, we use a graph convolution-based placer to learn the optimized mapping between circuit connectivity and physical wirelength, and further decode the physical locations of nodes (i.e., the optimized initial placement solutions).
% To this end, we use low-frequency graph filter to eliminate the high-frequency components in graph signals, to enhance the smoothness of these signals, thereby obtaining optimized initial placement solutions.
Modern analytical placers view the placement problem as a nonlinear optimization process, often resulting in lengthy iteration times. 
To accelerate this process, we use a graph convolution-based placer to efficiently produce optimized placement results. 
This placer is an in-house version similar to the work~\cite{graphplanner}, and focuses on optimizing the placement by minimizing total wirelength and reducing overlap among components. 
Essentially, the goal is to establish an optimized mapping that correlates circuit connectivity with the physical locations of nodes.
Our approach utilizes the graph convolution-based technique not only to learn this optimized mapping between circuit connectivity and physical wirelength but also to decode and determine the optimized initial physical locations of the nodes. 
This method streamlines the placement process, efficiently translating connectivity data into practical, spatially aware placement solutions \textcolor{red}{(need callback to what does it mean to the mapper? What does it enable?)}.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{algorithm}[h]
    \caption{pigMAP-Placer Algorithm}
    \label{alg:aigplace}
    \begin{algorithmic}[1]
    \REQUIRE An AIG $\mathbb{A}$
    \ENSURE Legalized placement result;
    \STATE A circuit netlist modeled by an undirected weighted graph $G = (V,E) \leftarrow$ FloorPlan($A$);
    \STATE Set initial locations $g$ of cells $v \in V$;
    \STATE {Locations of movable cells $g_m \sim N(0,1)$ are placed at the center of the placement region;}
    \STATE Fixed cells are set at their predetermined locations;
    \STATE Compute optimized cell locations $g'$ using graph-convolution-based placer;
    \STATE {Input $g'$ to subsequent placer to complete placement task;}
    \RETURN The legalized placement result.
    \end{algorithmic}
\end{algorithm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The process of our AIG-Placer is detailed in Algorithm~\ref{alg:aigplace}. 
Initially, the AIG $A$ is modeled as a circuit netlist of minimal size by incorporating technology library. 
The procedure begins with a simulated floorplanning stage. 
Here, nodes represent gates and the core area dynamically scales based on the AIG size.
PIs and POs are designated as I/O and are assigned fixed positions along the perimeter of the simulated core to maintain structural integrity with the original AIG. 
Intermediate nodes, however, remain flexible in their placement (Line 1).
Subsequently, we convert the circuit netlist into a weighted graph $G$ using a clique net model~\cite{aigpl}. The AIG placer then processes this graph to generate optimized cell locations $g'$ (Lines 2-5). 
These optimized locations $g'$ serve as the starting point for the analytical placer, which significantly reduces the iteration time required to finalize the placement (Lines 6-7).

\begin{ownexample}
\label{exam1}
    Fig.\ref{fig:aig2} illustrates the random initial cell locations. 
    Due to our placer’s capability to bypass the time-consuming initialization phase and efficiently drive the placement process, it significantly cuts down the total runtime. 
    The final cell placements are showcased in Fig.~\ref{fig:aig6}.
    \textcolor{red}{Add a few sentences give an intuition what happened. Like the graph planner gradually adjust the locations so that the overall wirelength (HPWL?) is minimized.}
\end{ownexample}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[h]
  \centering  %图片全局居中
  \subfigbottomskip=5pt %两行子图之间的行间距
  % \subfigcapskip=-5pt %设置子图与子标题之间的距离
  \subfigure[AIG network of C17]{
    \label{fig:aig1}
    \includegraphics[width=0.45\linewidth]{latex/Fig/aig1.png}}
    \hspace{20mm}
  \subfigure[random initial cell locations]{
    \label{fig:aig2}
    \includegraphics[width=0.44\linewidth]{latex/Fig/aig2.png}}
    \subfigure[final cell locations]{
    \label{fig:aig6}
    \includegraphics[width=0.44\linewidth]{latex/Fig/aig6.png}}
  \caption{Example for AIG placement of benchmark C17.}
  \label{fig:aig}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{pigMAP-Mapper: placement-aware mapping}
\label{subsec:pigMAP}
The placement-aware mapping algorithm is detailed in Algorithm~\ref{alg:paflow}.
Considering that the logic function of each matched gate can be inverted by adding an inverter, we compute across both signal phases (Line 2).
The algorithm initiates by setting four crucial metrics, critical path wirelength ($wl$), total wirelength ($total_{wl}$), critical path delay ($delay$), and area ($area_f$), to $\infty$
%to provide a baseline for optimization 
 (Line 3). 
 Afterwards, mapper computes approximate position of all supergates by calculating the average position of pins associated with their corresponding cuts, 
 utilizing ``\texttt{compute\_position}'' function (Line 5).
% \textcolor{red}{As the algorithm enumerates cuts and supergates, it begins by computing their approximate positions using the ``\texttt{compute\_position}'' function.}
% \textcolor{red}{This step involves} calculating the average position of the pins associated with each cut (Algorithm~\ref{alg:search_pins}).
% \textcolor{red}{(Instead of saying this computation is vital because... a long sentence. Just say The average positions is associated with the cuts and are used in the future wirelength computation steps.)}
The resultant position-supergate tuples are stored to enable future wirelength computation.

Intending to find the best match for the visiting node, 
the mapper enumerates all possible supergate and compute their metrics, including current delay ($current\_delay$), area flow ($current\_area\_f$), and two distinct wirelength metrics :$current\_wl$ and $current\_total\_wl$ (Lines 6-10).
$current\_wl$ denotes the maximum wirelength formulated for performance-driven optimization \textcolor{red}{need confirmed}, defined in Def.~\ref{def2},
whereas $total\_wl$ is the total wirelength formulated for power-driven optimization \textcolor{red}{need confirmed}, define in Def.~\ref{def3}.
% Further, the algorithm matches supergates to nodes and computes the wirelength to accessible PIs using Manhattan distance, defined by the absolute value of the coordinate differences (Lines 6-10). 
In this context, the performance-driven strategy focuses on reducing the maximum wirelength, whereas the power-driven strategy aims to minimize the total circuit wirelength.

% Following the wirelength computations, constraint-aided pruning is employed to accelerate the match selection process. 
Following metrics computation, we employ constraint-aided pruning to accelerate match selection,
removing matches that fail to meet the required arrival times or exceed maximum wirelength constraints. 
Under a pigMAP-Performance strategy, the mapper primarily focuses on the weighted sum of arrival time and maximum wirelength. 
Conversely, in the pigMAP-Power strategy, after discarding matches with excessive arrival times, total wirelength is prioritized, emphasizing reduction of power consumption (Lines 13-17).
In scenarios where gates exhibit similar timing performance due to delay and wirelength comparison, the algorithm advances to compare additional parameters such as area and cut size successively. 
Moreover, the power-driven mapping includes a global area flow consideration to address potential area increases that could result from wirelength optimizations, recognizing that excessive area also contributes to higher power consumption.
Ultimately, a thorough comparison of these parameters identifies the best-performing supergate for each node ($n_i$), which is then saved for future reference. 
This saved supergate aids in subsequent wirelength computations when a higher-level node accesses node $n_i$, ensuring optimized placement based on these strategic evaluations (Lines 18-19).

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{algorithm}[t]
    \caption{Placement-aware Mapping Algorithm.}
    \label{alg:paflow}
    \begin{algorithmic}[1]
    \REQUIRE Optimization strategy $\mathbb{S}$, AIG $\mathbb{A}$, target node $n$
    \ENSURE Data structure of mapping $\mathbb{M}$
    \FORALL{none PI node $n$ of $\mathbb{A}$ in topological order}
        \FORALL{phase}
            \STATE $wl, total\_wl, delay, area \gets \infty$;
            \FORALL{$cut$ of $n$}
                \STATE $\mathbb{P}$= \texttt{computePosition}($cut$)
                \FORALL{$gate$ in \texttt{supergate}($cut$)}
                    \STATE $current\_delay \gets $ \texttt{compute\_delay}($n, gate, cut$);
                    \STATE $current\_area\_f \gets$ \texttt{compute\_area}($n, gate, cut$);
                    \STATE $current\_wl \gets$ \texttt{compute\_wl}($n, gate, cut$);
                    \STATE $current\_total\_wl \gets$ \texttt{compute\_wl}($n, gate, cut$);
                    \IF{\texttt{setConstraint}($\mathbb{S}$)}
                        \STATE \textbf{continue};
                    \ENDIF
                    \IF{\texttt{comparePara}()}
                        \STATE $total\_wl \gets current\_total\_wl$;
                        \STATE $wl \gets current\_wl$;
                        \STATE $best\_gate \gets gate$;
                        \STATE $delay \gets current\_delay$;
                        \STATE $area\_f \gets current\_area\_f$;
                    \ENDIF
                \ENDFOR
            \ENDFOR
            \IF{\texttt{comparePara}()}
                \STATE \texttt{matchSel}($n$, $wl$, $total\_wl$, $best\_gate$, $delay$, $area$);
            \ENDIF
        \ENDFOR
    \ENDFOR
    \RETURN $map$;
    \end{algorithmic}
\end{algorithm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\textcolor{red}{Eq \ref{eq:maxwl} and Eq \ref{eq:totalwl} need to explain. Similar to Eq 1}

\subsubsection{Performance-driven model:}
\label{subsubsec:per}
Suppose the mapper is visiting node $n_i$, its cut is $c_i$, and its matched supergate is $sg_i$.
Leaves of $n_i$ in order $l^\text{th}$ are $n_{i,l}$, and their respective cut and matched supergate are $c_{i,l}$ and $sg_{i,l}$.
The coordinates of supergate $sg_i$ are $sg_i.x$, $sg_i.y$.
The maximum wirelength of $sg_i$ is defined as follow,
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{owndefinition} \textbf{Maximum wirelength:} Maximum wirelength of supergate $sg\_i$ is maximum wirelength among all paths set off from $sg\_i$ to every accessible PI.
    \label{def2}
    \begin{equation}
        \label{eq:maxwl}
        \text{MW}(sg_i)=\max_{0<i<l} |sg_i.x-sg_{i,l}.x|+|sg_i.y-sg_{i,l}.y|+\text{MW}(sg_{i,l}).
    \end{equation}
    $\text{MW}(sg_{i,l})$ in Equation~\ref{eq:maxwl} is the maximum wirelength of the best supergate matched for node $n_{i,l}$ in preceding iterations.
\end{owndefinition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsubsection{Power-driven model:}
\label{subsubsec:pow}
The total wirelength from the visiting node to the PIs is computed by aggregating the discounted wirelength of all paths accessed by leaf nodes.
The total wirelength is defined as TW($sg_i$), 
\begin{owndefinition} \textbf{Total wirelength:} Total wirelength is 
    \label{def3}
    \begin{small}
    \begin{equation}
    \label{eq:totalwl}
        \text{TW}(sg_i)=\sum_{0<i<l} |sg_i.x-sg_{i,l}.x|+|sg_i.y-sg_{i,l}.y|+\text{TW}(sg_{i,l})/\text{ERef}
    \end{equation}
    \end{small}
    The discount factor ``ERef'' accounts for the reference estimation of node $n_{i,l}$, helping to prevent redundant calculations of total wirelength for circuits with multiple fan-outs. 
\end{owndefinition}
This strategy ensures that while striving for efficiency in wirelength and power, the overall area remains controlled, aligning the design more closely with the desired power optimization objectives.

\textcolor{red}{Can you add some explain of the matching algorithm here? I can understand there are different costs, and you probably use the similar algorithm from ABC. But here does not explain how to go from a weifhted graph to a mapped netlists} 

\begin{ownexample}
\label{exam2}
    In Fig.\ref{fig:aig1}, when selecting the best cut for node $8$, different strategies can significantly impact the decision.
    As for delay mode, cut \{$2,7$\} and cut \{$2,3,4$\} are analyzed to determine which one results in the worst delay. 
    The cut that exhibits the least delay is chosen as the optimal cut. 
    In performance-driven mode, We compare the wirelength of node \{$8$\} to nodes \{$2,7$\} for cut \{$2,7$\} and nodes \{$7,8$\} to nodes \{$2,3,4$\} for cut \{$2,3,4$\}.
    The wirelength is evaluated without exceeding the worst delay.
    In power-driven mode, when node $8$ is the fan-in of multiple nodes (e.g., nodes $9$ and $11$), the worst wirelength for node $8$ is divided by 2. 

    \textcolor{red}{Add something about which gates they are mapped to, and what decision is made in this process.}
\end{ownexample}
